Impact of Spatial Frequency Based Constraints on Adversarial Robustness

Adversarial examples mainly exploit changes to input pixels to which humans are not sensitive to, and arise from the fact that models make decisions based on uninterpretable features. Interestingly, cognitive science reports that the process of interpretability for human classification decision relies predominantly on low spatial frequency components. In this paper, we investigate the robustness to adversarial perturbations of models enforced during training to leverage information corresponding to different spatial frequency ranges. We show that it is tightly linked to the spatial frequency characteristics of the data at stake. Indeed, depending on the data set, the same constraint may results in very different level of robustness (up to 0.41 adversarial accuracy difference). To explain this phenomenon, we conduct several experiments to enlighten influential factors such as the level of sensitivity to high frequencies, and the transferability of adversarial perturbations between original and low-pass filtered inputs.

==> table/cifar10_svhn_Lhigh.tex <==
\begin{table}
\caption{CIFAR10 and SVHN. Accuracy on clean ($Acc$) and adversarial examples ($Acc_{adv}$) of models trained with loss $L^{high}_i$}
\begin{center}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\multicolumn{6}{c}{\textbf{CIFAR10}}\\
\hline
& \multicolumn{5}{c}{Filtering intensity (loss $L^{high}_i$)}\\
& \textit{2} & \textit{4} & \textit{6} & \textit{8} & \textit{10} \\ 
\hline
$Acc$ & 0.92 & 0.92 & 0.86 & 0.87 & 0.86\\
$Acc_{adv}$ & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
\hline
\multicolumn{6}{c}{\textbf{SVHN}}\\
\hline
& \multicolumn{5}{c}{Filtering intensity (loss $L^{high}_i$)}\\
& \textit{2} & \textit{4} & \textit{6} & \textit{8} & \textit{10} \\ 
\hline
$Acc$ & 0.96 & 0.95 & 0.95 & 0.95 & 0.95\\
$Acc_{adv}$ & 0.21 & 0.17 & 0.11 & 0.08 & 0.06\\
\hline
\end{tabular}
}
\end{center}
\label{cifar10_svhn_Lhigh}
\end{table}

==> table/cifar10_svhn_Llow.tex <==
\begin{table}
\caption{CIFAR10 and SVHN. Accuracy on clean ($Acc$) and adversarial examples ($Acc_{adv}$) of models trained with loss $L^{low}_i$}
\begin{center}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\multicolumn{6}{c}{\textbf{CIFAR10}}\\
\hline
& \multicolumn{5}{c}{Filtering intensity (loss $L^{low}_i$)}\\
& \textit{2} & \textit{4} & \textit{6} & \textit{8} & \textit{10} \\  
\hline
$Acc$ & 0.74 & 0.84 & 0.85 & 0.90 & 0.92\\
$Acc_{adv}$ & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
\hline
\multicolumn{6}{c}{\textbf{SVHN}}\\
\hline
& \multicolumn{5}{c}{Filtering intensity (loss $L^{low}_i$)}\\
& \textit{2} & \textit{4} & \textit{6} & \textit{8} & \textit{10} \\ 
\hline
$Acc$ & 0.93 & 0.96 & 0.96 & 0.96 & 0.96\\
$Acc_{adv}$ & 0.06 & 0.26 & 0.41 & 0.29 & 0.0\\
\hline
\end{tabular}
}
\end{center}
\label{cifar10_svhn_Llow}
\end{table}

==> table/constrained_loss_cifar10.tex <==
\begin{table}
\caption{CIFAR10. Best and worst accuracy on clean ($Acc$) and adversarial examples ($Acc_{adv}$) of models trained with the constrained loss $L^{freq}_{i,j} (i: low, j:high)$. For $i=0$ $L^{freq}$ is noted $L^{high}_{j}$ and for $j=0$ $L^{freq}$ is noted $L^{low}_{i}$ }
\begin{center}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c|c}
\multicolumn{5}{c}{\textbf{CIFAR10}}\\
\hline
& \textit{$Acc$} & \textit{$Constraints$} & \textit{$Acc_{adv}$} & \textit{$Constraints$} \\  
\hline
Best & 0.95 & $L^{freq}_{5,3}$, $L^{freq}_{8,6}$ & 0.12 & $L^{freq}_{5,3}$\\
Worst & 0.74 & $L^{low}_{2}$ & 0.0 & $L^{low}_{*}$, $L^{high}_{*}$\\
\hline
\end{tabular}
}
\end{center}
\label{cifar10_Lfreq}
\end{table}

==> table/constrained_loss_cifar10_svhn_simnet.tex <==
\begin{table}
\caption{CIFAR10, SVHN, Small ImageNet. Best and worst accuracy on clean ($Acc$) and adversarial examples ($Acc_{adv}$) of models trained with the constrained loss $L^{freq}_{i,j}$.} %For $i=0$ $L^{freq}$ is noted $L^{high}_{j}$ and for $j=0$ $L^{freq}$ is noted $L^{low}_{i}$ }
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|cc}
\multicolumn{5}{c}{\textbf{CIFAR10}}\\
\hline
& \textit{$Acc$} & \textit{$Constraints$} & \textit{$Acc_{adv}$} & \textit{$Constraints$} \\  
\hline
Best & 0.95 & $L^{freq}_{5,3}$, $L^{freq}_{8,6}$ & 0.12 & $L^{freq}_{5,3}$\\
Worst & 0.74 & $L^{low}_{2}$ & 0.0 & $L^{low}_{*}$, $L^{high}_{*}$\\
\hline

\multicolumn{5}{c}{\textbf{SVHN}}\\

\hline
& \textit{$Acc$} & \textit{$Constraints$} & \textit{$Acc_{adv}$} & \textit{$Constraints$} \\  
\hline
Best & 0.96 & $L^{low}_{i>2}$ & 0.41 & $L^{low}_{6}$\\
Worst & 0.93 & $L^{low}_{2}$ & 0.0 & $L^{low}_{*}$, $L^{freq}_{10,4}$, $L^{freq}_{6,10}$, , $L^{freq}_{6,8}$\\
\hline

\multicolumn{5}{c}{\textbf{Small ImageNet}}\\
\hline
& \textit{$Acc$} & \textit{$Constraints$} & \textit{$Acc_{adv}$} & \textit{$Constraints$} \\  
\hline
Best & 0.92 & $L^{freq}_{60,10}$ & 0.36 & $L^{freq}_{40,20}$\\
Worst & 0.89 & $L^{freq}_{10,60}$ & 0.0 & $L^{freq}_{60,10}$, $L^{freq}_{10,4}$, $L^{freq}_{6,10}$, , $L^{freq}_{6,8}$\\
\hline
\end{tabular}
}
\end{center}
\label{cifar10_svhn_simnet_Lfreq}
\end{table}








==> table/constrained_loss_simnet.tex <==
\begin{table}
\caption{Small ImageNet. Best and worst accuracy on clean ($Acc$) and adversarial examples ($Acc_{adv}$) of models trained with the constrained loss $L^{freq}_{i,j} (i: low, j:high)$. For $i=0$ $L^{freq}$ is noted $L^{high}_{j}$ and for $j=0$ $L^{freq}$ is noted $L^{low}_{i}$ }
\begin{center}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c|c}
\multicolumn{5}{c}{\textbf{Small ImageNet}}\\
\hline
& \textit{$Acc$} & \textit{$Constraints$} & \textit{$Acc_{adv}$} & \textit{$Constraints$} \\  
\hline
Best & 0.92 & $L^{freq}_{60,10}$ & 0.36 & $L^{freq}_{40,20}$\\
Worst & 0.89 & $L^{freq}_{10,60}$ & 0.0 & $L^{freq}_{60,10}$, $L^{freq}_{10,4}$, $L^{freq}_{6,10}$, , $L^{freq}_{6,8}$\\
\hline
\end{tabular}
}
\end{center}
\label{simnet_Lfreq}
\end{table}

==> table/constrained_loss_svhn.tex <==
\begin{table}
\caption{SVHN. Best and worst accuracy on clean ($Acc$) and adversarial examples ($Acc_{adv}$) of models trained with the constrained loss $L^{freq}_{i,j} (i: low, j:high)$. For $i=0$ $L^{freq}$ is noted $L^{high}_{j}$ and for $j=0$ $L^{freq}$ is noted $L^{low}_{i}$ }
\begin{center}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c|c|c}
\multicolumn{5}{c}{\textbf{SVHN}}\\
\hline
& \textit{$Acc$} & \textit{$Constraints$} & \textit{$Acc_{adv}$} & \textit{$Constraints$} \\  
\hline
Best & 0.96 & $L^{low}_{i>2}$ & 0.41 & $L^{low}_{6}$\\
Worst & 0.93 & $L^{low}_{2}$ & 0.0 & $L^{low}_{*}$, $L^{freq}_{10,4}$, $L^{freq}_{6,10}$, , $L^{freq}_{6,8}$\\
\hline
\end{tabular}
}
\end{center}
\label{svhn_Lfreq}
\end{table}

==> table/transferability_all_v2.tex <==
\begin{table}
\caption{CIFAR10, SVHN and Small ImageNet. Transferability results (adversarial accuracy). Base denotes a natural model.}
\begin{subtable}{1.0\linewidth}
\begin{center}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c||c|c|c|c|c|c}
\multicolumn{7}{c}{\textbf{CIFAR10}}\\
\hline
& \multicolumn{6}{c}{Filtering intensity ($i$)}\\
& \textit{2} & \textit{4} & \textit{6} & \textit{8} & \textit{10} & \textit{12} \\  
\hline
$Base \rightarrow M^{low}_{i}$ & 0.91 & 0.86 & 0.73 & 0.48 & 0.31 & 0.24\\
$M^{low}_i \rightarrow Base$ & 0.97 & 0.82 & 0.87 & 0.66 & 0.39 & 0.22\\
\hline
$Base \rightarrow M^{high}_{i}$ & 0.0 & 0.02 & 0.13 & 0.13 & 0.13 & 0.06\\
$M^{high}_i  \rightarrow Base$ & 0.19 & 0.44 & 0.81 & 0.88 & 0.9 & 0.95\\
\hline
\end{tabular}
}
\end{center}

\end{subtable}
\begin{subtable}{1.0\linewidth}
\begin{center}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c||c|c|c|c|c|c}
\multicolumn{7}{c}{\textbf{SVHN}}\\
\hline
& \multicolumn{6}{c}{Filtering intensity ($i$)}\\
& \textit{2} & \textit{4} & \textit{6} & \textit{8} & \textit{10} & \textit{12} \\  
\hline
$Base \rightarrow M^{low}_{i}$ & 0.95 & 0.77 & 0.44 & 0.24 & 0.19 & 0.21\\
$M^{low}_i \rightarrow Base$ & 0.96 & 0.54 & 0.32 & 0.26 & 0.13 & 0.19\\
\hline
$Base \rightarrow M^{high}_{i}$ & 0.25 & 0.13 & 0.21 & 0.16 & 0.21 & 0.13\\
$M^{high}_i \rightarrow Base$ & 0.31 & 0.96 & 0.99 & 1.0 & 1.0 & 1.0\\
\hline
\end{tabular}
}
\end{center}
\end{subtable}

\begin{subtable}{1.0\linewidth}
\begin{center}
\resizebox{0.87\linewidth}{!}{
\begin{tabular}{c||c|c|c|c|c}
\multicolumn{6}{c}{\textbf{Small ImageNet}}\\
\hline
& \multicolumn{5}{c}{Filtering intensity ($i$)}\\
& \textit{5} & \textit{10} & \textit{15} & \textit{20} & \textit{40} \\ 
\hline
$Base \rightarrow M^{low}_{i}$ & 0.92 & 0.88 & 0.82 & 0.76 & 0.63 \\
$M^{low}_i \rightarrow Base$ & 0.94 & 0.88 & 0.81 & 0.71 & 0.56 \\
\hline
$Base \rightarrow M^{high}_{i}$ & 0.46 & 0.49 & 0.47 & 0.46 & 0.57 \\
$M^{high}_i \rightarrow Base$ & 0.69 & 0.79 & 0.83 & 0.87 & 0.94 \\
\hline
\end{tabular}
}
\end{center}
\end{subtable}
\label{cifar10_svhn_smallImnet_transferability}
\end{table}
